Chorus: a Programming Framework for Building Scalable Differential Privacy Mechanisms

Differential privacy is fast becoming the gold standard in enabling statistical analysis of data while protecting the privacy of individuals. However, practical use of differential privacy still lags behind research progress because research prototypes cannot satisfy the scalability requirements of production deployments. To address this challenge, we present Chorus, a framework for building scalable differential privacy mechanisms which is based on cooperation between the mechanism itself and a high-performance production database management system (DBMS). We demonstrate the use of Chorus to build the first highly scalable implementations of complex mechanisms like Weighted PINQ, MWEM, and the matrix mechanism. We report on our experience deploying Chorus at Uber, and evaluate its scalability on real-world queries.

==> background.tex <==
\section{Background: Differential Privacy}

% \paragraph{Background}

This section summarizes the differential privacy concepts necessary
for the rest of the paper. We refer the reader to Dwork and
Roth~\cite{dwork2014algorithmic} for a comprehensive resource on
differential privacy.

Differential privacy provides a formal guarantee of
\emph{indistinguishability}: a differentially private result does not
yield very much information about which of two neighboring databases
was used in calculating the result. 
This guarantee is defined in terms of a \emph{privacy budget} $\epsilon$ (the smaller the budget, the stronger the guarantee).
The formal definition of differential privacy
is written in terms of the \emph{distance} $d(x,y)$ between two
databases, which represents the number of entries on which they differ: $d(x,y) = |\{i
: x_i \neq y_i\}|$.

\begin{definition}[Differential privacy]
A randomized mechanism $\mathcal{K} : D^n \rightarrow
\mathbb{R}^d$ preserves $(\epsilon, \delta)$-differential privacy if
for any pair of databases $x, y \in D^n$ such that $d(x,y) = 1$, and
for all sets $S$ of possible outputs:

\[\mbox{Pr}[\mathcal{K}(x)\in S] \leq e^\epsilon
  \mbox{Pr}[\mathcal{K}(y) \in S] + \delta \]
\end{definition}

One measure of sensitivity is \emph{global sensitivity}, which is the maximum difference between
the query's result on \emph{any} two possible databases with distance 1:

% Intuitively,
% the sensitivity of a query corresponds to the amount its results can
% change when the database changes.

\begin{definition}[Global Sensitivity] For $f:D^n \rightarrow
  \mathbb{R}^d$ and all $x,y \in D^n$, the global sensitivity of $f$
  is
  
\[GS_f = \max_{x,y:d(x,y)=1}||f(x)-f(y)||\]
\end{definition}

The Laplace mechanism~\cite{dwork2006calibrating} is one of the
simplest general-purpose differential privacy mechanisms. It adds
noise to the output of a function $f : D^n \rightarrow \mathbb{R}^d$
scaled to $GS_f / \epsilon$, and provides $\epsilon$-differential
privacy.


% For a true database $x$, the Laplace mechanism releases $f(x) + (Y_1,
% ..., Y_d)$, where the $Y_i$ are drawn i.i.d. from $\mbox{Lap}(GS_f /
% \epsilon)$. This mechanism is $\epsilon$-differentially private, but
% for some queries (including those with joins), the global sensitivity
% is unbounded, which makes releasing accurate results impossible.

\begin{comment}
Another definition of sensitivity is \emph{local
  sensitivity}~\cite{dwork2009differential,nissim2007smooth}, which 
is the maximum difference between the query's results on the
\emph{true database} and any neighbor of it:

\begin{definition}[Local Sensitivity] For $f:D^n \rightarrow
  \mathbb{R}^d$ and $x \in D^n$, the local sensitivity of $f$ at $x$
  is
  
\[LS_f(x) = \max_{y:d(x,y)=1}||f(x)-f(y)||\]
\end{definition}

Local sensitivity is often much
lower than global sensitivity since it is a property of the single true
database rather than the set of all possible databases.

\paragraph{Smoothing functions}
Because local sensitivity is based on the true database, it must
be used carefully to avoid leaking information about the data.
Prior work~\cite{nissim2007smooth,dwork2009differential}
describes techniques for using local sensitivity to enforce differential privacy.
Henceforth we use the term \emph{smoothing functions} to refer to
these techniques. Smoothing functions are independent of the method used
to compute local sensitivity, but generally require that local
sensitivity can be computed an arbitrary distance $k$ from the true
database (i.e. when at most $k$ entries are changed):

% Two prior techniques allow the use of local
% sensitivity without leaking information: smooth sensitivity~\cite{nissim2007smooth}
% and propose-test-release (PTR)~\cite{dwork2009differential}.
% Henceforth we use the term \emph{smoothing function} to refer to
% these techniques. Both require the ability to determine the local
% sensitivity of a query at an arbitrary distance $k$ from the true
% database (i.e. when at most $k$ entries are changed).

% \begin{definition}[Local Sensitivity at Distance] The local
%   sensitivity of $f$ at distance $k$ from the true database $x$ is:
  
% \[A_f^{(k)}(x) =\max_{y \in D^n:d(x,y) \leq k}LS_f(y)\]
% \end{definition}

\begin{definition}[Local Sensitivity at Distance]
  The local sensitivity of $f$ at distance $k$ is:
  
  \[A_f^{(k)}(x) =\max_{y \in D^n:d(x,y) \leq k}LS_f(y)\]  
  % $$
  % \begin{array}{ll}
  %   S^*_{f,\epsilon}(x) & = \max_{k=0,1,...,n} e^{-k \epsilon} (\max_{y \in D^n:d(x,y) \leq k}LS_f(y))\\
  %   & = \max_{k=0,1,...,n} e^{-k \epsilon} A_f^{(k)}(x)\\
  % \end{array}
  % $$
\end{definition}
\end{comment}
% \noindent The value of $A_f^{(k)}(x)$ is then used to define a
% \emph{$\beta$-smooth upper bound on local sensitivity}, which can be
% used with the Laplace mechanism to produce differentially private
% results.

% Propose-test-release follows a three-step
% process: (1) the analyst \emph{proposes} a sensitivity $b$; (2) the
% system performs a differentially private \emph{test} to check that the
% true database is ``far'' from one with local sensitivity higher than
% $b$; (3) if the test passes, the results of the query are
% \emph{released} with Laplace noise scaled to $b/\epsilon$. Smooth
% sensitivity smooths the actual local sensitivity using nearby local
% sensitivities to eliminate its potential to leak information. Smooth
% sensitivity avoids the rapid changes possible in local sensitivity,
% and can be used directly in the Laplace mechanism.

% \begin{definition}[Smooth Sensitivity]
%   The smooth sensitivity for a query $f$ with privacy budget
%   $\epsilon$ is:

%   \[S^*_{f,\epsilon}(x) = \max_{k=0,1,...,n} e^{-k \epsilon} A_f^{(k)}(x)\]
%   % $$
%   % \begin{array}{ll}
%   %   S^*_{f,\epsilon}(x) & = \max_{k=0,1,...,n} e^{-k \epsilon} (\max_{y \in D^n:d(x,y) \leq k}LS_f(y))\\
%   %   & = \max_{k=0,1,...,n} e^{-k \epsilon} A_f^{(k)}(x)\\
%   % \end{array}
%   % $$
% \end{definition}


% the amount that the query's output can change when a single row
% of the \emph{true database} is changed. Similarly, the local
% sensitivity of a query $f$ at distance $k$ is the maximum local
% sensitivity achievable by changing $k$ rows in the true database.
% % Unlike the query's global
% % sensitivity, which captures the change in the query's output given
% % \emph{any two} databases, the local sensitivity fixes one of the two
% % to be the true database on which the query is to run and considers all
% % possible single-row changes to that database.

% \begin{definition}[Local Sensitivity] For $f:D^n \rightarrow
%   \mathbb{R}^d$ and $x \in D^n$, the local sensitivity of $f$ at $x$ is
% \[LS_f(x) = \max_{y:d(x,y)=1}||f(x)-f(y)||\]
% \end{definition}
% \begin{definition}[Local Sensitivity at Distance] The local
%   sensitivity of $f$ at distance $k$ is:
% \[A_f^{(k)}(x) =\max_{y \in D^n:d(x,y) \leq k}LS_f(y)\]
% \end{definition}

% \paragraph{Propose-test-release \& Smooth Sensitivity}
% %
% Propose-test-release (PTR)~\cite{dwork2009differential} and smooth
% sensitivity~\cite{nissim2007smooth} are two mechanisms for using local
% sensitivity without leaking information. PTR follows a three-step
% process: (1) the analyst \emph{proposes} a sensitivity $b$; (2) the
% system performs a differentially private \emph{test} to check that the
% true database is ``far'' from one with local sensitivity higher than
% $b$; (3) if the test passes, the results of the query are
% \emph{released} with Laplace noise scaled to $b/\epsilon$. Smooth
% sensitivity smooths the actual local sensitivity using nearby local
% sensitivities to eliminate its potential to leak information. Smooth
% sensitivity avoids the rapid changes possible in local sensitivity,
% and can be used directly in the Laplace mechanism.
% \begin{definition}[Smooth Sensitivity]
%   The smooth sensitivity for a query $f$ with privacy budget
%   $\epsilon$ is:
%   \rmspcsm
%   \[S^*_{f,\epsilon}(x) = \max_{k=0,1,...,n} e^{-k \epsilon} A_f^{(k)}(x)\]
%   % $$
%   % \begin{array}{ll}
%   %   S^*_{f,\epsilon}(x) & = \max_{k=0,1,...,n} e^{-k \epsilon} (\max_{y \in D^n:d(x,y) \leq k}LS_f(y))\\
%   %   & = \max_{k=0,1,...,n} e^{-k \epsilon} A_f^{(k)}(x)\\
%   % \end{array}
%   % $$
% \end{definition}
% \rmspc


% \subsection{Background: Differential Privacy}

% %  At the same time, differential privacy mechanisms attempt to
% % maximize utility for queries that do not depend too much on any
% % individual, so that trends in the dataset can be revealed even while
% % individual privacy is protected.

% % Differential privacy has a number of features that make it a good fit
% % for protecting individual privacy at organizations. First, it applies equally
% % well across employees and teams with different requirements; since it
% % protects individual privacy directly, it does not require a
% % per-employee or per-team security policy to be written. Second,
% % differential privacy is immune to attacks based on auxiliary
% % knowledge, allowing each query to be treated individually without
% % considering the existing knowledge of the query's submitter. Third,
% % differential privacy provides several knobs for tuning the tradeoff
% % between privacy and utility, allowing companies to customize the solution
% % to provide the accuracy required by its analysts while meeting its
% % privacy requirements. No matter the settings of these knobs,
% % differential privacy provides a formal guarantee of the level of
% % privacy provided.

% Differential privacy ensures that the results of a query do not depend
% too much on the presence or absence of any individual in the
% dataset. A differential privacy \emph{mechanism} is a randomized
% algorithm for computing differentially private results. One such
% mechanism is the \emph{Laplace mechanism}~\cite{dwork2006calibrating},
% which involves computing a statistical function (or query) $f$ of the
% database, then adding noise to the results drawn from the Laplacian
% distribution. The magnitude of the noise is scaled based on the
% \emph{global sensitivity} of $f$, which is the maximum difference
% $||f(x)-f(y)||$ between the results of $f$ on any two databases $x$
% and $y$ that differ in at most one row.

% The global sensitivity of a query with joins is unbounded, because
% changing a single row could cause an unbounded number of new matches
% with a particular join key. \emph{Local
%   sensitivity}~\cite{nissim2007smooth} provides a tighter bound by
% taking into account the actual database on which $f$ runs: the local
% sensitivity of $f$ is the maximum difference $||f(x)-f(y)||$ where $x$
% is the actual database instance (or \emph{true database}) and $y$ is
% any database differing from $x$ in one row.

% Because it is based on the true database, the local sensitivity of a
% query can actually leak information about the database, and must be
% applied carefully. Two mechanisms for doing so are
% propose-test-release (PTR)~\cite{dwork2009differential} and smooth
% sensitivity~\cite{nissim2007smooth}. In addition to the query's local
% sensitivity, these two mechanisms require computing the local
% sensitivity at various \emph{distances} from the true database.

% % Both can be used to calculate an
% % effective sensitivity that does not leak information about the
% % database, and this effective sensitivity can be used with the Laplace
% % mechanism to make the query's results differentially private.





==> more-examples.tex <==
\section{Additional Examples}
\label{sec:additional-examples}

\begin{figure}
\begin{lstlisting}
WITH
  __orig_query AS (
    with
  dim_driver as (select *, 1 as weight from dim_driver),
  fact_trip as (select *, 1 as weight from fact_trip)
SELECT
  "count"(*) "__col_0"
, "isnull"("sum"("weight"), 0) "__col_0_w"
FROM
  (
   WITH
     r1_norms AS (
      SELECT
        "driver_uuid"
      , "isnull"("sum"("weight"), 0) "r1norm"
      FROM
        dim_driver
      GROUP BY "driver_uuid"
   ) 
,    r2_norms AS (
      SELECT
        "driver_uuid"
      , "isnull"("sum"("weight"), 0) "r2norm"
      FROM
        fact_trip
      GROUP BY "driver_uuid"
   ) 
,    all_norms AS (
      SELECT
        "r1_norms"."driver_uuid" "key"
      , ("r1norm" + "r2norm") "norm"
      FROM
        (r1_norms
      INNER JOIN r2_norms ON (("r1_norms"."driver_uuid" = "r2_norms"."driver_uuid")))
   ) 
   SELECT
     "r1"."signup_city_id" "__join_col_2"
   , "r2"."uuid" "__join_col_1"
   , (("r1"."weight" * "r2"."weight") / "norm") "weight"
   FROM
     ((dim_driver r1
   INNER JOIN fact_trip r2 ON (("r1"."driver_uuid" = "r2"."driver_uuid")))
   INNER JOIN all_norms n ON (("r1"."driver_uuid" = "n"."key")))
)  ALIAS_HERE
WHERE ("__join_col_2" = 1)

)
, __uniform_samples AS (
   SELECT
    ("random"() - 0.5) "__uniform___col_0"

   , *
   FROM
     __orig_query
)
, __laplace_samples AS (
   SELECT
    (-(1.0 / 0.1) * (CASE WHEN ("__uniform___col_0" < 0) THEN -1.0 ELSE 1.0 END)) * "ln"((1 - (2 * "abs"("__uniform___col_0")))) "__laplace___col_0"

   , *
   FROM
     __uniform_samples
)
SELECT
   ("__col_0_w" + "__laplace___col_0") "count"

FROM
  __laplace_samples
\end{lstlisting}

  \caption{Example query, transformed into an intrinsically private query via WPINQ}
  \label{fig:example-wpinq}
\end{figure}


==> proofs.tex <==
\section{Proofs}
\label{sec:proofs-semant-pres}

\paragraph{Proof of Theorem~\ref{thm:composition_block} (composition).}
\begin{proof}
  Assume that $\rightarrow_a$ and $\rightarrow_b$ preserve semantics,
  and $Q \rightarrow_a Q' \rightarrow_b Q''$. We have that: (1) $Q:U$,
  $Q':U$, and $Q:U''$ \om{Typo.}; (2) $|Q| = |Q'| = |Q''|$; and (3) $Q$, $Q'$,
  and $Q''$ contain the same logical attributes. Thus by
  Definition~\ref{def:shape-pres}, $\rightarrow_c$ preserves
  semantics.
\end{proof}

\paragraph{Proofs of semantic preservation for individual mechanisms.}
\begin{theorem}%[Laplace Noise preserves semantics]
  The Laplace Noise transformation (Figure~\ref{fig:laplace-noise})
  satisfies the semantic preservation property.
  % For all queries $Q$ and $Q'$, if $Q \arrlap Q'$, then (1)
  % the set of output columns is preserved: $Q: U \Rightarrow Q': U$,
  % and (2) the number of output rows is preserved: $|Q| = |Q'|$.
  \label{thm:lap_block}
\end{theorem}

\begin{proof}
  The rules in Figure~\ref{fig:laplace-noise} define only one
  transformation, at the top level of the query. The $\Unif$ function
  adds a column $u_x$ for each original column $x$; the $\Lap$
  function consumes this column, replacing the original column $x$
  with its original value plus a value sampled from the Laplace
  distribution. The outermost projection produces exactly the same set
  of attributes as the input query $Q$, preserving the schema; the
  transformation adds only projection nodes, so the number of output
  rows is preserved; no join or select can occur at the top level of a
  query, so no logical attributes are modified.
\end{proof}

\begin{theorem}%[Metadata Propagation preserves semantics]
  The Metadata Propagation transformation (Figure~\ref{fig:metadata})
  satisfies the semantic preservation property.
  % For all queries $Q$ and $Q'$, if $Q \arr Q'$, then (1)
  % the set of output columns is preserved: $Q: U \Rightarrow Q': U$,
  % and (2) the number of output rows is preserved: $|Q| = |Q'|$.
  \label{thm:metadata_block}
\end{theorem}

\begin{proof}
  The only rules that make major modifications to the original query
  are those for joins and counts. The other rules add a new attribute
  $\meta$ and propagate it through the query, but do not change the
  number or contents of the rows of any relation. At the top level of
  the query (i.e. $q \in Q$), the transformation eliminates the
  attribute $\meta$. For queries without joins or subquery
  aggregations, the Metadata Propagation transformation is the
  identity transformation, so it satisfies semantic preservation.

  We argue the remaining cases by induction on the structure of $Q$.

  \case{Case $r_1 \underset{A = B}{\bowtie} r_2$} Let $r = r_1
  \underset{A = B}{\bowtie} r_2$. If $\update$ does not change the
  query's semantics, except to update the attribute $\meta$ (i.e. $r:U
  \Rightarrow r = \Pi_{U-m} \update(r)$), then the semantics of $r$ are
  preserved.

  \case{Case $\id{Count}(r)$ and $\id{Count}_{G_1..G_n}(r)$} The rule
  modifies the $\meta$ attribute, but does not modify any other
  attribute or change the size of the relation, so semantics are
  preserved.
\end{proof}

\begin{theorem}%[Replacing Aggregation Functions preserves semantics]
  The Replace Aggregation Function transformation
  (Figure~\ref{fig:aggfn}) satisfies the semantic preservation
  property.
  % For all queries $Q$ and $Q'$, if $Q \arr Q'$,
  % then (1) the set of output columns is preserved: $Q: U \Rightarrow
  % Q': U$, and (2) the number of output rows is preserved: $|Q| =
  % |Q'|$.
  \label{thm:aggfn_block}
\end{theorem}

\begin{proof}
  Aggregation function replacement has the potential to modify the
  values of the query's results, but not its shape or logical attributes. The
  transformation's only rule allows changing one function to another,
  but preserves the grouping columns and number of functions. The
  schema, number of rows, and logical attributes are therefore preserved.
\end{proof}

\begin{theorem}[Subsampling preserves semantics]
  If the aggregation function $\agg$ aggregates over the $\meta$
  attribute, then our Subsampling transformation
  (Figure~\ref{fig:sampling}) satisfies the semantic preservation
  property.
  % For all queries $Q$ and $Q'$ and aggregation
  % functions $\agg$, if $Q \arrsamp Q'$ and $\agg$ aggregates over the
  % $\meta$ column, then (1) the set of output columns is preserved: $Q:
  % U \Rightarrow Q': U$, and (2) the number of output rows is
  % preserved: $|Q| = |Q'|$.
  \label{thm:samp_block}
\end{theorem}

\begin{proof}
  We know that $Q$ has the form $\id{Count}(r)$ or
  $\underset{G_1..G_n, m}{\id{Count}}(r)$.
  % 
  By Theorem~\ref{thm:metadata_block}, we know that in either case, if
  $r \arr r'$, then $r$ has the same semantics as $r'$. We proceed by
  cases.

  \case{Case $Q = \id{Count}(r)$} Let $q_1 =
  \id{Count}_{\meta}(r')$. By the definition of the transformation,
  $Q' = \agg(q_1)$. The query $q_1$ has exactly one row per unique
  value of $\meta$. Since $\agg$ aggregates over $\meta$, $\agg(q_1)$
  has exactly one row, and therefore preserves the semantics of $Q$.

  \case{Case $Q = \underset{G_1..G_n, m}{\id{Count}}(r)$} Let
  $q_1 = \underset{G_1..G_n, m}{\id{Count}}(r')$. By the
  definition of the transformation, $Q' = \agg(q_1)$. The query $q_1$
  has exactly one row per unique tuple $(G_1..G_n, \meta)$. Since
  $\agg$ aggregates over $\meta$, $\agg(q_1)$ has exactly one row per
  unique tuple $(G_1..G_n)$, and therefore preserves the semantics of $Q$.

\end{proof}


==> rewriting-algorithm-proofs.tex <==

\subsubsection{Proofs: Algorithm Correctness for Differential Privacy Mechanisms}

This section provides proofs that each of our intrinsically private
queries is a faithful implementation of the corresponding differential
privacy mechanism. The algorithm correctness property states that
the output of an intrinsically private query $Q'$ is equal to the
output of running the corresponding differential privacy mechanism
on the original (non-private) query $Q$. We formalize and prove this
property for each mechanism independently, because the mechanisms
differ in their semantics.

\begin{theorem}[Elastic Sensitivity]
  \label{thm:elastic-sensitivity}
  The output of $Q'$ is equal to the output of running $Q$ using the
  Elastic Sensitivity mechanism~\cite{allegro}.
\end{theorem}

\begin{proof}
  Elastic Sensitivity~\cite{allegro} defines a method for calculating
  an upper bound on the smooth sensitivity of $Q$, then calls for
  applying the Laplace mechanism with this sensitivity to enforce
  differential privacy.

  By construction, $Q'$ applies the Laplace mechanism using the
  Elastic Sensitivity of $Q$. The two projection operations wrapping
  $Q$ apply to each cell in turn, adding noise scaled to the
  sensitivity specified by Elastic Sensitivity.
\end{proof}

\begin{theorem}[Restricted Sensitivity]
  \label{thm:restricted-sensitivity}
  The output of $Q'$ is equal to the output of running $Q$ using the
  Restricted Sensitivity
  mechanism~\cite{Blocki:2013:DPD:2422436.2422449}.
\end{theorem}

\begin{proof}
  Same as Theorem~\ref{thm:elastic-sensitivity}.
\end{proof}

\begin{theorem}[Weighted PINQ]
  \label{thm:wpinq}
  The output of $Q'$ is equal to the output of running $Q$ using the
  Weighted PINQ mechanism~\cite{proserpio2014calibrating}.
\end{theorem}

\begin{proof}
  The WPINQ mechanism~\cite{proserpio2014calibrating} executes queries
  on \emph{weighted datasets}. A traditional dataset is a collection
  of rows; in a weighted dataset, each row additionally carries a
  weight. A counting query on a traditional dataset returns the number
  of rows satisfying a condition; the corresponding query on a
  weighted dataset returns the \emph{sum of the weights} of the rows
  satisfying the condition.

  Proserpio et al.~\cite{proserpio2014calibrating} define a
  \emph{noisy count} aggregation function that performs a
  differentially private counting query on a weighted dataset. They
  additionally define an equation (reproduced in
  Equation~\eqref{eqn:wpinq_join}) for scaling the weights of each
  record in such a dataset when the query performs a join.

  Our intrinsically private query must (1) correctly implement
  weighted datasets; (2) correctly implement counting queries over
  weighted datasets; and (3) correctly implement scaling of weights
  for joins.

  To satisfy condition (1), our transformation uses the Metadata
  Propagation building block to add an attribute $\meta$, initializing
  the weight of each record to 1. To satisfy condition (2), our
  transformation uses the Replace Aggregation Function building block
  to replace counting queries with a sum of weights (i.e. a sum of the
  $\meta$ attribute). To satisfy condition (3), our transformation
  defines the $\update$ function given to the Metadata Propagation
  building block based on Equation~\eqref{eqn:wpinq_join}, as defined
  by Proserpio et al.~\cite{proserpio2014calibrating}. Finally, our
  transformation adds Laplace noise scaled to 1, as required by the
  WPINQ mechanism.
\end{proof}

\begin{theorem}[Sample \& Aggregate]
  \label{thm:wpinq}
  The output of $Q'$ is equal to the output of running $Q$ using the
  Sample \& Aggregate mechanism~\cite{nissim2007smooth,smith2011privacy}.
\end{theorem}

\begin{proof}
  We assume that $\agg$ implements Widened Winsorized mean as defined
  in Algorithm 1 of Smith~\cite{smith2011privacy}. Our intrinsically
  private query must implement Algorithm 3 of
  Smith~\cite{smith2011privacy}. That algorithm has three steps: (1)
  divide the database randomly into chunks, (2) run the input function
  (i.e. the query) on each chunk), and (3) run Widen Winsorized mean
  to aggregate the chunked results.

  Our intrinsically private query implements the same algorithm. The
  Subsampling building block divides the database randomly (step 1) and
  executes the query on each chunk (step 2). The Widened Winsorized
  mean (step 3) is accomplished by the aggregation function $\agg$.
\end{proof}



==> rewriting-building-blocks.tex <==
\section*{Formalization \& Correctness}
\label{sec:building-blocks}

This section formalizes the construction of intrinsically private
queries as introduced in Section~\ref{sec:intr-priv-quer-1}. We begin by introducing notation. We then define reusable transformation rules that can be composed to
construct mechanisms. Next, we formalize the four mechanisms described
earlier in terms of these rules. 
% Finally, we prove a correctness
% property: our transformations do not modify the semantics of the input
% query (Section~\ref{sec:corr-prop}).

% By formalizing the transformation rules separately from the individual
% mechanisms, we allow the rules to be re-used in defining new
% mechanisms---taking advantage of the common algorithmic requirements
% demonstrated in Table~\ref{fig:mechanisms}. An additional benefit of
% this approach is the ability to prove correctness properties of the
% rules themselves, so that these properties extend to all mechanisms
% implemented using the rules.

% These transformations may also be useful in implementing new
% mechanisms beyond the four discussed in this paper.

\subsection*{Preliminaries}
\label{sec:preliminaries}

\paragraph{Core relational algebra.}
We formalize our transformations as rewriting rules on a core
relational algebra that represents general statistical queries.
We define the core relational algebra in
Figure~\ref{fig:core-relational-algebra}. This algebra includes the
most commonly-used features of query languages like SQL: selection
($\sigma$), projection ($\Pi$), equijoins ($\bowtie$), and counting
with and without aggregation. We also include several features
specifically necessary for our implementations: constant values,
random numbers, and the arithmetic functions \emph{ln}, \emph{abs},
and \emph{sign}.

We use standard notation for relational algebra with a few
exceptions. We extend the projection operator $\Pi$ to attribute
expressions, which allows projection to add new named columns to a
relation. For example, if relation $r$ has schema $U$, then the
expression $\Pi_{U \cup \mbox{weight}:1}r$ adds a new column named
``weight'' with the default value 1 for each row to the existing columns in
$r$. In addition, we combine aggregation and grouping, 
writing $\underset{a_1..a_n}{\id{Count}}$ to indicate a counting aggregation
with grouping by columns $a_1..a_n$. We write
$\underset{a_1..a_n}{\id{Sum}_a}$ to indicate summation of column $a$,
grouping by columns $a_1..a_n$.

% \todo{limitations}

% \todo{citation for where we got this notation}

\paragraph{Notation for rewriting rules.}
Each transformation is defined as a set of inference rules that
rewrites a relational algebra expression. A particular rule allows
rewriting an expression as specified in its conclusion (below the
line) if the conditions specified in its antecedent (above the line)
are satisfied (either through syntactic properties of the query or by
applying another inference rule).
%\todo{cite something about the syntax of inference rules}

Our approach relies on the ability to analyze and
rewrite SQL queries. This rewriting can be achieved by a
rule-based query optimization engine~\cite{calcite,GPORCA}. 
\tocut{Note, however, that in
contrast to traditional query optimization rules, our transformations
are \emph{deterministic}---for each relational algebra expression,
exactly one rule applies, and the rules are defined recursively. Our
rules can therefore be implemented as a recursive function, without
the complexity of a complete rule-oriented optimizer.}

Most of the conditions specified in our rewriting rules use standard
notation. One exception is conditions of the form $Q : U$, which we
use to denote that the query $Q$ results in a relation with schema
$U$. We extend this notation to denote the schemas of database tables
(e.g. $t : U$) and relational expressions (e.g. $r_1 : U$).

Some of our rewriting rules have global parameters, which we denote by
setting them above the arrow indicating the rewriting rule itself. For
example, $r \overset{x}{\rightarrow} \Pi_x r$ allows rewriting $r$ to
project only the column named $x$, where the value of $x$ is provided
as a parameter. Most parameters are values, but parameters can also be
functions mapping a relational algebra expression to a new
expression. For example, $r \overset{f}{\rightarrow} f(r)$ indicates
rewriting $r$ to the result of $f(r)$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Syntax
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
  \ruleFontSize
  
  
  $$
  \begin{array}{lcl}
    \multicolumn{3}{l}{\cellcolor{gray!15}\mbox{Attribute expressions}}\\
    a & & \emph{attribute name}\\
    e & ::= & a \;|\; a:v \\
    v & ::= & a \;|\; n \in \mathbb{N} \;|\; v_1 + v_2 \;|\; v_1 * v_2 \;|\; v_1 / v_2\\
      & | & \id{rand}() \;|\; \id{randInt}(n) \;|\; \id{ln}(v) \;|\; \id{abs}(v) \;|\; \id{sign}(v) \\
    
    \\[-2mm] 
    % \multicolumn{3}{l}{\cellcolor{gray!15}\mbox{Aggregation expressions \& functions}}\\ 
    % E & ::= & \textit{fun}(a) \\
    % \textit{fun} & ::= & \textsf{count} \;|\; \textsf{avg} \;|\; \textsf{sum} \\
    % & | & \textsf{max} \;|\; \textsf{min}\\
    % \\
    \multicolumn{3}{l}{\cellcolor{gray!15}\mbox{Relational transformations}}\\ 
    R & ::= & t \;|\; R_1 \underset{x = y}{\bowtie} R_2 \;|\; \Pi_{e_1, ..., e_n} R \;|\; \sigma_\varphi R \vspace*{1mm}\\
      & | & \id{Count}(R) \;|\; \underset{a_1..a_n}{\id{Count}}(R) \\
    \\[-2mm]
    
    \multicolumn{3}{l}{\cellcolor{gray!15}\mbox{Selection predicates}}\\
    \varphi & ::= & e_1 \theta e_2 \;|\; e \theta v\\
    \theta & ::= & < \;|\; \leq \;|\; = \;|\; \neq \;|\; \geq \;|\; >\\
    \\[-2mm]
    
    \multicolumn{3}{l}{\cellcolor{gray!15}\mbox{Queries}}\\ 
    Q & ::= & \id{Count}(R) \;|\; \underset{a_1..a_n}{\id{Count}}(R) 
    %& | & 
    \;|\; \id{Sum}_a (R) \;|\; \underset{a_1..a_n}{\id{Sum}_a} (R) 
  \end{array}
  $$

  
%   \newcommand{\mbar}{\;\mid\;}
%   $$
% \begin{array}{l c l}
%   Q &::=& R \mbar \{t\} \mbar \sigma_\theta(Q) \mbar \pi_U(Q) \mbar
%           Q_1 \underset{A = B}{\bowtie} Q_2 \\
%   & | &  Q_1 \times Q_2 \mbar Q_1 \cup Q_2 \mbar \rho_{A \mapsto B}(Q)\\
%   & | &  G_1, ..., G_m \; g_{f_1(A_1), ..., f_n(A_n)}(Q)\\

%   U &::=& A \mbar A: e\\
  
%   e &::=& A \mbar n \mbar \mbox{rand()} \mbar e_1 \;\textit{op}\; e_2 \mbar \mbox{ln}(e) \mbar \mbox{abs}(e) \mbar \mbox{sgn}(e)\\

%   \textit{op} &::=& + \mbar - \mbar * \mbar /\\
%   \end{array}
%   $$
  \rmspc
  \rmspc
  \caption{Syntax of core relational algebra}
  \label{fig:core-relational-algebra}
\end{figure}

\subsection*{Transformation Rules}
\label{sec:transformation-rules}

\paragraph{Laplace Noise.}
All four mechanisms in Table~\ref{fig:mechanisms} require generating
noise according to the Laplace distribution. We accomplish this task
using the \emph{Laplace Noise} transformation, defined in
Figure~\ref{fig:laplace-noise}. This transformation has one parameter:
$\gamma$, which defines the scale of the noise to be added to the
query's result. For a query with sensitivity 1 and privacy budget
$\epsilon$, for example, $\gamma = 1/\epsilon$ suffices to enforce
differential privacy.

The Laplace Noise transformation defines a single inference rule. This
rule allows rewriting a top-level query with schema $U$ according to
the $\Lap$ function. $\Lap$ wraps the query in two projection
operations; the first (defined in $\Unif$) samples the uniform
distribution for each value in the result, and the second (defined in
$\Lap$) uses this value to add noise drawn from the Laplace
distribution.

%\input{transformation-figures/laplace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Laplace Noise
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
  \small
  \vspace*{-2mm}
  $$
  \begin{array}{c}
    \fbox{$Q \arrlap Q$}
    \quad \quad
  \inference
    {Q:U}{Q \arrlap \Lap(Q)}
    \\[2mm]
    \begin{aligned}
      \mbox{where}&\\
    \Unif(Q) &= \Pi_{U \cup \{\metu_x : \id{rand}() - 0.5 | x \in U\}}(Q))\\
      \Lap(Q) &= \Pi_{\{x : x + - \gamma\, \id{sign}(\metu_x) \id{ln}(1 - 2\, \id{abs}(\metu_x)) | x \in U \}}(\Unif(Q))\\

    \end{aligned}
  \end{array}
  $$
  \rmspc
  \caption{Laplace Noise Transformation}\label{fig:laplace-noise}
\end{figure}


\paragraph{Metadata Propagation.}
Many mechanisms require tracking metadata about each
row as the query executes. To accomplish this, we define the
\emph{Metadata Propagation} transformation in
Figure~\ref{fig:metadata}. The Metadata Propagation transformation
adds a column to each referenced table and initializes its value for
each row in that table, then uses the specified composition functions
to compose the values of the metadata column for each resulting row of
a join or an aggregation.

The Metadata Propagation transformation has three parameters: $\init$,
a function defining the initial value of the metadata attribute for
each row in a database table; $\update$, a function specifying how to
update the metadata column for a join of two relations; and
$\countupdate$, a function specifying how to update the metadata
column for subqueries.

The inference rule for a table $t$ uses projection to add a new
attribute to $t$'s schema to hold the metadata, and initializes that
attribute to the value of $\init()$. The rules for projection and
selection simply propagate the new attribute.
%
% The rule for joins first renames the metadata attribute $\meta$ in the
% two relations being joined, and performs the join. Then, the rule
% forms the new schema for the joined relation by removing the old
% metadata attributes ($\meta_1$ and $\meta_2$) from the joined relation
% and adding a new metadata attribute whose value is determined by the
% update function $\update$.
The rule for joins applies the $\update$ function to perform a
localized update of the metadata column.
%
The rules for counting subqueries invoke the update function
$\countupdate$ to determine the new value for the metadata attribute.
%
Finally, the rules for counting queries eliminate the metadata
attribute to preserve the top-level schema of the query.

% \input{transformation-figures/metadata}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Metadata
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[t]
\vspace*{-5mm}
\ruleFontSize  
  $$
  \begin{array}{c}
    \fbox{$R \arr R$}
    \quad 

    \inference{r_1 \arr r_1' \quad r_2 \arr r_2' \quad r_1':U_1 \quad r_2':U_2}
    {r_1 \underset{A = B}{\bowtie} r_2 \arr \update(r_1' \underset{A = B}{\bowtie} r_2')}
    % {\begin{gathered} r_1 \underset{A = B}{\bowtie} r_2 \arr \\
    %     \Pi_{(U_1 -\meta_1) \cup (U_2 - \meta_2) \cup (\meta : \meta'(A))}
    %     (\rho_{\meta \mapsto \meta_1}(r_1') \underset{A = B}{\bowtie} \rho_{\meta \mapsto \meta_2}(r_2')) \\
    %     \mbox{where } \meta'(k) = \update(r_1, r_2, \meta_1, \meta_2, A, B, k)
    %   \end{gathered}}

    \\[\sepmm]
    \inference
    {t:U \quad \meta \not \in U}{t \arr \Pi_{U \cup \meta : \init()} t}

    \quad

    \inference{r \arr r'}
    {\Pi_U(r) \arr \Pi_{U \cup \{\meta\}}(r')}
    
    \\[\sepmm]
    
    % \inference{A \neq \meta \quad r \arr r'}
    % {\rho_{A \mapsto B}(r) \arr \rho_{A \mapsto B}(r')}

%    \id{Count}(R) \;|\; \id{Count}_{G_1..G_n}(R)


    \inference{r \arr r'}
    {\sigma_\phi(r) \arr \sigma_\phi(r')}

    \quad
    
    \inference{r \arr r' \quad \id{Count}(r') : U}
    {\id{Count}(r) \arr \Pi_{U \cup \meta : \countupdate(r') } \id{Count}(r')}

    \\[\sepmm]

    \inference{r \arr r' \quad \underset{a_1..a_n}{\id{Count}}(r') : U}
    {\underset{a_1..a_n}{\id{Count}}(r) \arr \Pi_{U \cup \meta : \countupdate(r') } \underset{a_1..a_n}{\id{Count}}(r')}


    % \inference{r \arr r'}
    % {\begin{gathered} G_1, ..., G_m \; g_{f_1(A_1), ..., f_n(A_n)}(r) \arr \\
    %   G_1, ..., G_m \; g_{f_1(A_1), ..., f_n(A_n)}(r') \end{gathered}}

    \\[\sepmm]
    \fbox{$Q \arr Q$}
     \quad %\quad
    %\hspace*{1mm}

    %\id{Count}(R) \;|\; \underset{G_1..G_n}{\id{Count}}(R)

    \inference{r \arr r'}
    {\id{Count}(r) \arr \id{Count}(r')}

    \\\\
    % \quad
    %\hspace*{1mm}

    \inference{r \arr r'}
    {\underset{a_1..a_n}{\id{Count}}(r) \arr \underset{a_1..a_n}{\id{Count}}(r')}
  \end{array}
  $$
  \rmspc \rmspc \rmspc \rmspc
  \caption{Metadata Propagation Transformation}\label{fig:metadata}
\end{figure}




\paragraph{Replacing Aggregation Functions.}
The \emph{Replace Aggregation Function} transformation, defined in
Figure~\ref{fig:aggfn}, allows replacing one aggregation function
($\Gamma$) with another ($\Gamma'$). To produce syntactically valid
output, $\Gamma$ and $\Gamma'$ must be drawn from the set of available aggregation functions. The antecedent is empty in the rewriting
rules for this transformation because the rules operate only on the outermost
operation of the query.

% This transformation is defined to replace counting
% queries with sums, but analogous rules can be added for other
% aggregation functions. The transformation has one parameter, $\delta$,
% which specifies the attribute to be summed. Its two rules simply
% replace the $\id{Count}$ function with a $\id{Sum}$ of the attribute
% $\delta$.

%\input{transformation-figures/aggfn}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Replace agg fn
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
  \ruleFontSize
  \vspace*{-5mm}
  $$
  \begin{array}{c}
    \fbox{$Q \arrrep Q$}
    \quad% \quad

    % \id{Count}(R) \;|\; \underset{G_1..G_n}{\id{Count}}(R)

    \inference{}
    {\Gamma(r) \arrrep \Gamma'(r)}

    \quad

    \inference{}
    {\underset{a_1..a_n}{\Gamma}(r) \arrrep \underset{a_1..a_n}{\Gamma'}(r)}

    
  % \inference
  %   {Q:U}
  %   {\begin{gathered} G_1, ..., G_m \; g_{f_1(A_1), ..., f_n(A_n)}(Q) \arrrep \\
  %       G_1, ..., G_m \; g_{\delta(f_1(A_1)), ..., \delta(f_n(A_n))}(Q) \end{gathered}}
  \end{array}
  $$
      \rmspc      \rmspc \rmspc \rmspc
  \caption{Replace Aggregation Function Transformation}
  \label{fig:aggfn}
  
\end{figure}


\paragraph{Subsampling.}
The \emph{Subsampling} transformation, defined in
Figure~\ref{fig:sampling}, splits the database into disjoint subsamples,
runs the original query on each subsample, and aggregates the results
according to a provided function. The Subsampling transformation is
defined in terms of the Metadata Propagation transformation, and can
be used to implement partition-based differential privacy mechanisms
like Sample \& Aggregate.

The parameters for the Subsampling transformation are $\agg$, a function
that aggregates the subsampled results, and $n$, the number of disjoint
subsamples to use during subsampling. Both inference rules defined by the
transformation rewrite the queried relation using the Metadata
Propagation transformation ($r \arr r'$). The parameters for Metadata
Propagation initialize the metadata attribute with a random
\emph{subsample number} between zero and $n$, and propagate the
subsample number over counting subqueries. The update functions for
joins and counting subqueries is undefined, because subsampling is
incompatible with queries containing these features.\footnote{Subsampling
  changes the semantics of joins, since join keys in separate
  partitions will be prevented from matching. It also changes the
  semantics of aggregations in subqueries, since the aggregation is
  computed within a single subsample.}
%
In order to satisfy the semantics preservation property, the aggregation
function $\agg$ must transform the query results on each subsample into a
final result with the same shape as the original query. Many
aggregation functions satisfy this property (e.g. the mean of all
subsamples), but not all of them provide  privacy.

%\input{transformation-figures/sample}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Subsampling
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
  \ruleFontSize
  $$
  \begin{array}{c}
    \fbox{$Q \arrsamp Q$}
    \quad \quad

    % \id{Count}(R) \;|\; \underset{G_1..G_n}{\id{Count}}(R)

    \inference{r \arr r'}
    {\id{Count}(r) \arrsamp \agg ( \underset{m}{\id{Count}}(r'))}

    \\[\sepmm]

    \inference{r \arr r'}
    {\underset{G_1..G_n}{\id{Count}}(r) \arrsamp \agg ( \underset{G_1..G_n, m}{\id{Count}}(r') )}

    \\\\
    \begin{aligned}
      \mbox{where } \init &= \id{randInt}(n),
      \update = \bot,
      \countupdate(r) = \bot,
       \mbox{and } \agg \mbox{ aggregates over } \meta
      
    \end{aligned}
    
  % \inference
  %   {Q:U}
  %   {\begin{gathered} G_1, ..., G_m \; g_{f_1(A_1), ..., f_n(A_n)}(Q) \arrrep \\
  %       G_1, ..., G_m \; g_{\delta(f_1(A_1)), ..., \delta(f_n(A_n))}(Q) \end{gathered}}
  \end{array}
  $$

  \rmspc \rmspc
  \caption{Subsampling Transformation}
  \label{fig:sampling}
  
\end{figure}

% \begin{figure}
%   \small
%   \vspace*{-2mm}
%   $$
%   \begin{array}{c}
%     \fbox{$Q \rightarrow Q$}
%     \quad \quad
%   \inference
%     {}{\It(q_f, q_1, \dots, q_k) \rightarrow q_f(q_1) \cup \dots \cup q_f(q_k)}
%   \end{array}
%   $$
%   \rmspc
%   \caption{Iteration Transformation}\label{fig:iteration}
% \end{figure}

% \begin{figure}
%   \small
%   \vspace*{-2mm}
%   $$
%   \begin{array}{c}
%     \fbox{$Q \rightarrow Q$}
%     \quad \quad
%   \inference
%     {}{\mbox{SVT}(T, q_1, \dots, q_k) \rightarrow q_f(q_1) \cup \dots \cup q_f(q_k)}
%   \end{array}
%   $$
%   \rmspc
%   \caption{SVT Transformation}\label{fig:svt}
% \end{figure}


\subsection*{Mechanism Definitions}
\label{sec:mech-defin}

We now formally define the mechanisms described earlier in terms of
our transformations. We describe each mechanism as
a series of one or more transformations, and define the parameters for
each transformation to obtain the correct semantics for the mechanism.

We describe Elastic Sensitivity, Restricted Sensitivity, Weighted
PINQ, and Sample \& Aggregate; the Exponential Mechanism and Sparse
Vector Technique can be encoded the same way, but require additional
constructs to be added to the relational algebra and cannot
transform queries written in the standard algebra.

\vspace*{3mm}
\begin{mdframed}[style=exampledefault,frametitle={Elastic Sensitivity}]
  Let $s$ be the Elastic Sensitivity of $Q$. Let
  $\gamma = s / \epsilon$. If $Q \arrlap Q'$, then $Q'$ is an
  intrinsically private query via Elastic Sensitivity.
  
  %\[Q \arrlap Q'\]
  
\end{mdframed}

\begin{mdframed}[style=exampledefault,frametitle={Restricted Sensitivity}]
  Let $s$ be the restricted
  sensitivity of $Q$. Let
  $\gamma = s / \epsilon$. If $Q \arrlap Q'$, then $Q'$ is an
  intrinsically private query via Restricted Sensitivity.
  
  %\[Q \arrlap Q'\]
  
\end{mdframed}

\begin{mdframed}[style=exampledefault,frametitle={Weighted PINQ}]
  \vspace*{4pt}
  Let $\init = 1$ and let $\update$ scale weights as described in
  Section~\ref{sec:weighted-pinq}. Let $\gamma = 1/\epsilon$. If $Q
  \arr Q' \arrrep Q'' \arrlap Q'''$, then $Q'''$ is an intrinsically
  private query via Weighted PINQ.

\end{mdframed}

\begin{mdframed}[style=exampledefault,frametitle={Sample \& Aggregate}]
\vspace*{4pt}
  Let $\agg$ implement private Winsorized
  mean~\cite{smith2011privacy} for a desired $\epsilon$. If $Q \arrsamp Q'$, then $Q'$ is an
  intrinsically private query via Sample \&
  Aggregate.
\end{mdframed}



\input{rewriting-proofs}




==> rewriting-proofs.tex <==
\subsection*{Correctness}
\label{sec:corr-prop}
\vspace*{-4mm}
The correctness criterion for a traditional query rewriting system is
straightforward: the rewritten query should have the same semantics
(i.e. return the same results) as the original query. For
intrinsically private queries, however, the definition of correctness
is less clear: enforcing differential privacy \emph{requires}
modifying the results to preserve privacy.

% We therefore define a relaxed notion of correctness, which we call
% \emph{semantic preservation}. Informally, semantic preservation is
% satisfied when (1) the transformed query has the same schema as the
% original query; (2) the transformed query has the same set of tuples
% as the original query; and (3) the transformation does not modify
% tuple values used to determine query logic (e.g. join keys or
% attributes used in filtering). Together, these properties ensure that
% the basic semantics of the query do not change, but allows adding new
% data or modifying attributes that are not involved in the query's
% logic (e.g. by adding noise). In Section~\ref{sec:corr-prop}, we
% formalize this notion and prove that our transformations satisfy it.



In this section, we define \emph{semantic preservation}, which formalizes the intuitive notion that our transformations should perturb the result attributes of the query, as required for enforcing differential privacy, but change nothing else about its semantics. Transformations should preserve the size and shape of
the query's output, and also its \emph{logical}
attributes---those which are used as
join keys or to perform filtering (i.e. the query makes decisions
based on these attributes).
%Each of our transformations preserve this property. Furthermore, 
Semantic preservation is preserved over composition of transformations, so semantic preservation holds for \emph{any} mechanism defined using our transformations.


% \paragraph{Definition of semantic preservation.}
% We begin by formalizing the desired property and showing that
% composing transformations preserves it. Semantic preservation holds
% when the transformation in question preserves the size and shape of
% the query's output, and additionally preserves its logical
% attributes. Logical attributes are those attributes which are used as
% join keys or to perform filtering (i.e. the query makes decisions
% based on these attributes, instead of simply outputting them).
% We begin
% by defining shape preservation formally and showing that
% transformations that satisfy the property can be composed without
% violating it. Then, we prove shape preservation for each building block.

\begin{definition}[Logical Attribute]
An attribute $a$ is a logical attribute if it appears as a join key in a join expression, in the filter condition $\varphi$ of a filter expression, or in the set of grouping attributes of a $\id{Count}$ or $\id{Sum}$ expression.
\end{definition}

\begin{definition}[Semantic Preservation]
  A transformation ($\rightarrow$) satisfies \emph{semantic preservation}
  if for all queries $Q$ and $Q'$, if $Q \rightarrow Q'$, then (1) the
  schema is preserved: $Q: U \Rightarrow Q': U$; (2) the number of
  output rows is preserved: $|Q| = |Q'|$; and (3) logical attributes
  are preserved (see Definition~\ref{def:logic-pres}).
  % no \emph{logical attribute}
  % (an attribute referenced in a join key or selection predicate) is modified by
  % the transformation.
  \label{def:shape-pres}
\end{definition}

\begin{definition}[Logical Attribute Preservation]
  Consider a transformation $Q:U \rightarrow Q':U$. Split $U$ into two
  sets of attributes $\{U_k, U_a\}$, such that $U_k$ contains all of
  the attributes from $U$ used as logical attributes in $Q$ and $U_a$ contains all of the other
  attributes. Now construct $Q'_r$ by renaming each attribute $k \in
  U_k$ in $Q'$ to $k'$. Then $\rightarrow$ preserves logical
  attributes if there exists a one-to-one relation $E \subseteq Q
  \times Q'_r$ such that for all $e \in E$ and $k \in U_k$, $e_k = e_{k'}$.
  \label{def:logic-pres}
\end{definition}

\ifvldb
\vspace*{-6mm}
\else
\fi

\begin{theorem}[Composition]
  If two transformations ($\rightarrow_a$ and $\rightarrow_b$) both
  satisfy semantic preservation, then their composition
  ($\rightarrow_c$) satisfies semantic preservation: for all queries
  $Q$, $Q'$, and $Q''$, if $Q \rightarrow_a Q' \rightarrow_b Q''$
  implies that $Q \rightarrow_c Q''$, and both $\rightarrow_a$ and
  $\rightarrow_b$ preserve semantics, then
  $\rightarrow_c$ preserves semantics.
  % For all queries $Q$ and $Q'$, if $Q \arrlap Q'$, then (1)
  % the set of output columns is preserved: $Q: U \Rightarrow Q': U$,
  % and (2) the number of output rows is preserved: $|Q| = |Q'|$.
  \label{thm:composition_block}
\end{theorem}

\ifextended
\begin{proof}
  Assume that $\rightarrow_a$ and $\rightarrow_b$ preserve semantics,
  and $Q \rightarrow_a Q' \rightarrow_b Q''$. We have that: (1) $Q:U$,
  $Q':U$, and $Q:U''$ \om{Typo.}; (2) $|Q| = |Q'| = |Q''|$; and (3) $Q$, $Q'$,
  and $Q''$ contain the same logical attributes. Thus by
  Definition~\ref{def:shape-pres}, $\rightarrow_c$ preserves
  semantics.
\end{proof}
\else
\fi


\ifextended
\begin{theorem}%[Laplace Noise preserves semantics]
  The Laplace Noise transformation (Figure~\ref{fig:laplace-noise})
  satisfies the semantic preservation property.
  % For all queries $Q$ and $Q'$, if $Q \arrlap Q'$, then (1)
  % the set of output columns is preserved: $Q: U \Rightarrow Q': U$,
  % and (2) the number of output rows is preserved: $|Q| = |Q'|$.
  \label{thm:lap_block}
\end{theorem}

\begin{proof}
  The rules in Figure~\ref{fig:laplace-noise} define only one
  transformation, at the top level of the query. The $\Unif$ function
  adds a column $u_x$ for each original column $x$; the $\Lap$
  function consumes this column, replacing the original column $x$
  with its original value plus a value sampled from the Laplace
  distribution. The outermost projection produces exactly the same set
  of attributes as the input query $Q$, preserving the schema; the
  transformation adds only projection nodes, so the number of output
  rows is preserved; no join or select can occur at the top level of a
  query, so no logical attributes are modified.
\end{proof}

\begin{theorem}%[Metadata Propagation preserves semantics]
  The Metadata Propagation transformation (Figure~\ref{fig:metadata})
  satisfies the semantic preservation property.
  % For all queries $Q$ and $Q'$, if $Q \arr Q'$, then (1)
  % the set of output columns is preserved: $Q: U \Rightarrow Q': U$,
  % and (2) the number of output rows is preserved: $|Q| = |Q'|$.
  \label{thm:metadata_block}
\end{theorem}

\begin{proof}
  The only rules that make major modifications to the original query
  are those for joins and counts. The other rules add a new attribute
  $\meta$ and propagate it through the query, but do not change the
  number or contents of the rows of any relation. At the top level of
  the query (i.e. $q \in Q$), the transformation eliminates the
  attribute $\meta$. For queries without joins or subquery
  aggregations, the Metadata Propagation transformation is the
  identity transformation, so it satisfies semantic preservation.

  We argue the remaining cases by induction on the structure of $Q$.

  \case{Case $r_1 \underset{A = B}{\bowtie} r_2$} Let $r = r_1
  \underset{A = B}{\bowtie} r_2$. If $\update$ does not change the
  query's semantics, except to update the attribute $\meta$ (i.e. $r:U
  \Rightarrow r = \Pi_{U-m} \update(r)$), then the semantics of $r$ are
  preserved.

  \case{Case $\id{Count}(r)$ and $\id{Count}_{G_1..G_n}(r)$} The rule
  modifies the $\meta$ attribute, but does not modify any other
  attribute or change the size of the relation, so semantics are
  preserved.
\end{proof}

\begin{theorem}%[Replacing Aggregation Functions preserves semantics]
  The Replace Aggregation Function transformation
  (Figure~\ref{fig:aggfn}) satisfies the semantic preservation
  property.
  % For all queries $Q$ and $Q'$, if $Q \arr Q'$,
  % then (1) the set of output columns is preserved: $Q: U \Rightarrow
  % Q': U$, and (2) the number of output rows is preserved: $|Q| =
  % |Q'|$.
  \label{thm:aggfn_block}
\end{theorem}

\begin{proof}
  Aggregation function replacement has the potential to modify the
  values of the query's results, but not its shape or logical attributes. The
  transformation's only rule allows changing one function to another,
  but preserves the grouping columns and number of functions. The
  schema, number of rows, and logical attributes are therefore preserved.
\end{proof}

\begin{theorem}[Subsampling preserves semantics]
  If the aggregation function $\agg$ aggregates over the $\meta$
  attribute, then our Subsampling transformation
  (Figure~\ref{fig:sampling}) satisfies the semantic preservation
  property.
  % For all queries $Q$ and $Q'$ and aggregation
  % functions $\agg$, if $Q \arrsamp Q'$ and $\agg$ aggregates over the
  % $\meta$ column, then (1) the set of output columns is preserved: $Q:
  % U \Rightarrow Q': U$, and (2) the number of output rows is
  % preserved: $|Q| = |Q'|$.
  \label{thm:samp_block}
\end{theorem}

\begin{proof}
  We know that $Q$ has the form $\id{Count}(r)$ or
  $\underset{G_1..G_n, m}{\id{Count}}(r)$.
  % 
  By Theorem~\ref{thm:metadata_block}, we know that in either case, if
  $r \arr r'$, then $r$ has the same semantics as $r'$. We proceed by
  cases.

  \case{Case $Q = \id{Count}(r)$} Let $q_1 =
  \id{Count}_{\meta}(r')$. By the definition of the transformation,
  $Q' = \agg(q_1)$. The query $q_1$ has exactly one row per unique
  value of $\meta$. Since $\agg$ aggregates over $\meta$, $\agg(q_1)$
  has exactly one row, and therefore preserves the semantics of $Q$.

  \case{Case $Q = \underset{G_1..G_n, m}{\id{Count}}(r)$} Let
  $q_1 = \underset{G_1..G_n, m}{\id{Count}}(r')$. By the
  definition of the transformation, $Q' = \agg(q_1)$. The query $q_1$
  has exactly one row per unique tuple $(G_1..G_n, \meta)$. Since
  $\agg$ aggregates over $\meta$, $\agg(q_1)$ has exactly one row per
  unique tuple $(G_1..G_n)$, and therefore preserves the semantics of $Q$.

\end{proof}

% See Appendix~\ref{sec:proofs-semant-pres} for the proofs of Theorems~\ref{thm:composition_block} and~\ref{thm:defin-semant-pres}.

\else
\begin{theorem}
Semantic preservation holds for the transformations defined in in
Section~\ref{sec:transformation-rules}, and thus for the every mechanism defined by composing these transformations.
\label{thm:defin-semant-pres}
\end{theorem}

% \proof
% \noindent See the extended version of this paper~\cite{chorus-arxiv-personal-webpage} for proofs of Theorems~\ref{thm:composition_block} and~\ref{thm:defin-semant-pres}.


\fi


  % individual proofs for each transformation.


% \paragraph{Semantic preservation holds for our transformations.}
% The remainder of this section contains proofs that semantic
% preservation holds for each of the transformations defined in
% Section~\ref{sec:transformation-rules}. As a direct consequence, the
% property also holds for every mechanism defined by composing these
% transformations.


==> selection.tex <==
% \begin{figure}
%   \centering
%     \scalebox{0.65}{
% \begin{forest} 
% mechanisms
% [Joins?, tikz={\draw[{Latex}-, thick] (.north) --++ (0,1);}
%     [Many-to-many\\joins?
%         [Elastic Sensitivity] 
%         [Restricted Sensitivity] 
%     ]   
%     [Counting\\query?
%         [PINQ]  
%         [Sample and Aggregate] 
%     ]   
% ] 
% \end{forest}
% }
% \smallskip

% \caption{Decision tree for automatic mechanism selection}
% \label{fig:mechanism_selection_decision_tree}
% \end{figure}

%\subsection{Mechanism Selection}
% %\label{sec:selection}
% The remainder of this section describes an example approach we have implemented based on syntactic properties of the query. As we show in Section~\ref{sec:selection_experiment}, this approach performs well on a real-world workload for the four mechanisms discussed in this paper.

% \tocut{This section describes how \system automatically selects a mechanism to execute an input query. Our approach uses known properties of the available mechanisms to select a mechanism that will support the input query and is likely to yield high utility. These properties are encoded in a set of extensible rules.}

%\paragraph{Syntax-Based Mechanism Selection.}
\paragraph{Mechanism selection.}
Our deployment of \system leverages a syntax-based selection procedure which aims to optimize for utility (low error). As we show in Section~\ref{sec:selection_experiment}, this approach performs well for this deployment. For different query workloads, other approaches may work significantly better, and \system is designed to support extension to these cases.

The syntax-based approach uses a set of rules that map SQL constructs supported by each mechanism to a heuristic scoring function indicating how likely queries using that construct will yield high utility.
%
For example, Restricted sensitivity~\cite{Blocki:2013:DPD:2422436.2422449} supports counting queries with joins, but does not support many-to-many joins. Elastic sensitivity~\cite{allegro} supports a wider set of equijoins, including many-to-many joins, but generally provides slightly lower utility than Restricted sensitivity due to smoothing. Sample \& aggregate~\cite{smith2011privacy} does not support joins, but does support additional aggregation functions (including ``average'' and ``median'').

% Weighted PINQ~\cite{proserpio2014calibrating} supports equijoins, including many-to-many joins, but is best suited for generating statistics for input to a separate post-processing step that is not automated. This mechanism is therefore not automatically selected by \system; the analyst may select WPINQ manually if he or she plans to perform the associated post-processing.

When a query is submitted, the mechanism selection engine analyzes the query to determine its syntactic properties including how many joins it has, of what type, and what aggregation functions it uses. It then applies the rules to determine which mechanisms can support the query and selects the mechanism with highest score. Note this process does not depend on the data and hence does not consume privacy budget.

This approach represents a simple but effective strategy for automatic mechanism selection. In Section~\ref{sec:selection_experiment}, we demonstrate that our rules are effective for selecting the best mechanism on a real-world query workload. This approach is also easily extended when a new mechanism is added: the mechanism designer simply adds new rules for SQL constructs supported by the mechanism. Moreover, the scoring function can be tuned for other objectives, for example favoring mechanisms achieving low performance overhead rather than highest utility.


==> system.tex <==
\section{The {\large \system} System}
\label{sec:system}

Intrinsically private queries enable the novel architecture of
\system, depicted in Figure~\ref{fig:sub2}. \system has three key
advantages compared to the strawman approach:

\begin{itemize}[topsep=1mm,leftmargin=4mm]
\itemsep1.0mm
\item \system supports a wide variety of differential privacy
  mechanisms coverage a range of algorithmic requirement
\item \system leverages any existing SQL database, eliminating data
  duplication and enabling scalability
\item \system has a single query submission and execution path,
  reducing complexity
\end{itemize}

\begin{figure}
  \centering
  \includegraphics[width=.50\textwidth]{figures/system_architecture}
  \caption{System architecture for \system}
  \label{fig:detailed-architecture}
\end{figure}

Figure~\ref{fig:detailed-architecture} summarizes the architecture of
the \system system. The system is designed around two major
components: analysis and rewriting. The \emph{rewriting engine}
provides a framework for transforming non-private SQL queries into
intrinsically private queries via transformation rules like those
defined earlier. The \emph{analysis engine} enables supporting static
analyses of the non-private query, such as determining its elastic
sensitivity. Adding a new differential privacy mechanism to \system
involves implementing the corresponding transformation rules using
\system's rewriting framework, and implementing any necessary analyses
using \system's analysis framework.

\paragraph{SQL analysis engine.} Some mechanisms require a static
analysis to determine properties of the input query. Computing elastic
sensitivity, for example, relies on a dataflow analysis of the
query. For these analyses, \system leverages Allegro, a dataflow
analysis framework for SQL queries.

\paragraph{Transformation engine.} To construct intrinsically private
queries from non-private input queries, \system contains a
transformation framework. Section~\ref{sec:intr-priv-quer-1} describes
the set of transformation rules required to construct intrinsically
private queries for the four mechanisms in
Table~\ref{fig:mechanisms}. Each set of rules is implemented in
\system using the framework provided by its transformation engine. The
framework is designed so that new mechanisms can be added easily, by
defining an analogous set of rules.

\todo{describe mechanism selection and the model}

\paragraph{Implementation.}
We have implemented \system in Java. The rewriting components required
for the four mechanisms discussed in this paper, plus the rewriting
framework itself, are implemented in just 1982 lines of code. For
static analysis, \system leverages the {\sc Allegro}
framework~\cite{allegro}. The analyses required for the four
mechanisms total 1083 lines of code.

